Mobile Head Tracking for eCommerce and Beyond

Shopping is difficult for people with motor impairments. This includes online shopping. Proprietary software can emulate mouse and keyboard via head tracking. However, such a solution is not common for smartphones. Unlike desktop and laptop computers, they are also much easier to carry indoors and outdoors.To address this, we implement and open source button that is sensitive to head movements tracked from the front camera of iPhone X. This allows developers to integrate in eCommerce applications easily without requiring specialized knowledge. Other applications include gaming and use in hands-free situations such as during cooking, auto-repair. We built a sample online shopping application that allows users to easily browse between items from various categories and take relevant action just by head movements. We present results of user studies on this sample application and also include sensitivity studies based on two independent tests performed at 3 different distances to the screen.

==> 0.abstract.tex <==
\begin{abstract}
%(148/150 words) Shopping is difficult for people with motor impairments and this includes online shopping due to the generalized user interfaces of devices. To form the easiest way of shopping, we built a mobile head-based online shopping application. We implemented UI buttons that are sensitive to head movements which tracking from the front camera of iPhone X. We also designed an integrated user interface with this method that allows users to easily browse between the items, select them by head and provides a hands-free online shopping experience. With this method, our user study shows that everyone can practice online shopping in an easy and enjoyable way without using hands. Beyond, the online shopping application, we actually propose open-source hands-free mobile UI components that will be available on the web and have potential to be integrated in any kind of mobile application that tends to provide hands-free interaction on mobile devices.
Shopping is difficult for people with motor impairments. This includes online shopping. Proprietary software can emulate mouse and keyboard via head tracking. However, such a solution is not common for smartphones. Unlike desktop and laptop computers, they are also much easier to carry indoors and outdoors.To address this, we implement and open source button that is sensitive to head movements tracked from the front camera of iPhone X. This allows developers to integrate in eCommerce applications easily without requiring specialized knowledge. Other applications include gaming and use in hands-free situations such as during cooking, auto-repair. We built a sample online shopping application that allows users to easily browse between items from various categories and take relevant action just by head movements. We present results of user studies on this sample application and also include sensitivity studies based on two independent tests performed at 3 different distances to the screen.

\end{abstract}
